Temporal Human Action Segmentation via Dynamic Clustering

We present an effective dynamic clustering algorithm for the task of temporal human action segmentation, which has comprehensive applications such as robotics, motion analysis, and patient monitoring. Our proposed algorithm is unsupervised, fast, generic to process various types of features, and applicable in both the online and offline settings. We perform extensive experiments of processing data streams, and show that our algorithm achieves the state-of-the-art results for both online and offline settings.

==> figure_overview.tex <==

\definecolor{babyblueeyes}{rgb}{0.63, 0.79, 0.95}


\definecolor{newgreen}{rgb}{0.53,0.66,0.42} % Define the color BrickRed

\begin{figure*}
\begin{center}

\begin{tikzpicture}[xscale=1,yscale=1,%rounded corners=3pt,
rknoten/.style={fill=jasper,color=jasper,draw=jasper,circle,scale=0.35},edge/.style={black, thick},
gknoten/.style={fill=newgreen,color=newgreen,draw=newgreen,circle,scale=0.35},edge/.style={black, thick},
bknoten/.style={fill=mblue,color=mblue,draw=mblue,circle,scale=0.35},edge/.style={black, thick},
redge/.style={draw=red!70,thick},
gedge/.style={draw=newgreen,thick},
bedge/.style={draw=newblue,thick},
edge/.style={black, thick}]




%%%% VGC16%%%%


\filldraw[fill=mblue!30, rounded corners=4pt] (2.7,0.7) rectangle (4.6,1.7);



\node at (3.65, 2.05) { \textbf{\footnotesize{Stage 1}}};

\node at (3.65, 1.35) { \textsf{\footnotesize{feature}}};
\node at (3.65, 1.05) {\textsf{\footnotesize{extraction}}};



\draw[mblue,  thick] (0,0) rectangle (2.5,1 ); 

\node at (1.25, 0.5) {\textsf{\footnotesize{raw data}}};


\draw[-stealth, line width=3pt, color=gray] (2.7,0.4) -- (4.6,0.4);


\begin{scope}[shift= {(4.8, 0)}]
\draw[mblue,  thick] (0,0) rectangle (2.5,1 ); 

 




\node at (0.1, -0.7) {\includegraphics[width=0.06\linewidth]{figures/idt_1}
};


\node at (1.2, -0.7) {\includegraphics[width=0.06\linewidth]{figures/idt_2}
};


\node at (2.3, -0.7) {\includegraphics[width=0.06\linewidth]{figures/idt_3}
};


\node at (0.1, -1.5) {\includegraphics[width=0.06\linewidth]{figures/idt_4}
};


\node at (1.2, -1.5) {\includegraphics[width=0.06\linewidth]{figures/idt_5}
};


\node at (2.3, -1.5) {\includegraphics[width=0.06\linewidth]{figures/idt_6}
};





\node at (1.25, 0.65) {\textsf{\footnotesize{temporally}}};

\node at (1.25, 0.35) {\textsf{\footnotesize{local feature}}};
\draw[-stealth, line width=3pt, color=gray] (2.7,0.4) -- (4.6,0.4);


\filldraw[fill=mblue!30, rounded corners=4pt] (2.7,0.7) rectangle (4.6,1.7);


\node at (3.65, 2.05) { \textbf{\footnotesize{Stage 2}}};


\node at (3.65, 1.35) { \textsf{\footnotesize{feature}}};
\node at (3.65, 1.05) {\textsf{\footnotesize{aggregation}}};


\end{scope}


\begin{scope}[shift= {(9.6, 0)}]
\draw[mblue,  thick] (0,0) rectangle (2.5,1 ); 
\draw[-stealth, line width=3pt, color=gray] (2.7,0.4) -- (4.6,0.4);

\node at (1.25, 0.5) {\textsf{\footnotesize{action patterns}}};

 
\filldraw[fill=mblue!30, rounded corners=4pt] (2.7,0.7) rectangle (4.6,1.7);


\node at (3.65, 2.05) { \textbf{\footnotesize{Stage 3}}};


\node at (3.65, 1.2) { \textsf{\footnotesize{clustering}}};


\end{scope}


\begin{scope}[shift= {(14.4, 0)}]
\draw[mblue,  thick] (0,0) rectangle (2.5,1 ); 

\node at (1.25, 0.5) {\textsf{\footnotesize{action clusters}}};

\end{scope}



\begin{scope}[xshift=14.3cm, yshift=-2.6cm]

\begin{scope}[xshift=0.2cm]
\draw[draw=gray, fill=white, opacity=0.9, thick] (1.95,1.73) ellipse (.45cm and .45cm);

\node[rknoten] (1) at (2.2,1.6){};
\node[rknoten] (2) at (2.2, 1.73){};

\node[rknoten] (2) at (1.99,2.){};
\node[rknoten] (3) at (2,1.7){};
\node[rknoten] (4) at (1.8,1.8){};

%\draw[redge] (1) -- (2);
%\draw[redge] (1) -- (3);
%\draw[redge] (1) -- (4);
%\draw[redge] (2) -- (3);
%\draw[redge] (2) -- (4);
%\draw[redge] (3) -- (4);
\end{scope}

\begin{scope}[rotate=50,xshift=-0.4cm,yshift=-1.5cm]
\draw[draw=gray, fill=white, opacity=0.9, thick] (2.15,0.75) ellipse (.45cm and .41cm);

\node[bknoten] (5) at (2.2,0.9){};
\node[bknoten] (6) at (2.4,0.7){};

\node[bknoten] (7) at (2.06,0.8){};
\node[bknoten] (7) at (2.1,0.6){};

\node[bknoten] (7) at (1.9,0.6){};
\node[bknoten] (8) at (2.22,0.45){};
%\draw[bedge] (5) -- (6);
%\draw[bedge] (5) -- (7);
%\draw[bedge] (5) -- (8);
%\draw[bedge] (6) -- (7);
%\draw[bedge] (6) -- (8);
%\draw[bedge] (7) -- (8);
\end{scope}



\begin{scope}[rotate=0,xshift=-1.1cm,yshift=-0.3cm]
\draw[draw=gray, fill=white, opacity=0.9, thick] (2,1.9) ellipse (.55cm and .45cm);
\node[gknoten] (9) at (1.9,2.2){};
\node[gknoten] (10) at (2.15,1.9){};
\node[gknoten] (11) at (1.8,1.8){};
\node[gknoten] (11) at (1.93,2.07){};

\node[gknoten] (12) at (2.15,2){};
\node[gknoten] (12) at (2.0,1.7){};

\node[gknoten] (13) at (2.25,1.7){};
%\draw[gedge] (9) -- (10);
%\draw[gedge] (9) -- (11);
%\draw[gedge] (9) -- (12);
%\draw[gedge] (9) -- (13);
%\draw[gedge] (10) -- (11);
%\draw[gedge] (10) -- (12);
%\draw[gedge] (10) -- (13);
%\draw[gedge] (11) -- (12);
%\draw[gedge] (11) -- (13);
%\draw[gedge] (12) -- (13);

\end{scope}


\end{scope}



\begin{scope}[xshift=9.7cm, yshift=-1.8cm]



\fill[newgreen,  thick] (0.05,0) rectangle (0.15,1.3 ); 

\fill[newgreen,  thick] (0.17,0) rectangle (0.27,1.1 ); 

\fill[newgreen,  thick] (0.29,0) rectangle (0.39,1 ); 


\fill[newgreen,  thick] (0.41,0) rectangle (0.51,0.7 ); 


\fill[newgreen,  thick] (0.53,0) rectangle (0.63,0.5 ); 

\fill[newgreen,  thick] (0.65,0) rectangle (0.75,0.76 ); 

\fill[newgreen,  thick] (0.77,0) rectangle (0.87,0.86 ); 


\fill[newgreen,  thick] (0.89,0) rectangle (0.99,0.99 ); 


\fill[newgreen,  thick] (1.01,0) rectangle (1.11,0.3 ); 

\fill[newgreen,  thick] (1.13,0) rectangle (1.23,0.35 ); 

\fill[newgreen,  thick] (1.25,0) rectangle (1.35,0.2 ); 

\fill[newgreen,  thick] (1.37,0) rectangle (1.47,0.67 ); 


\fill[newgreen,  thick] (1.49,0) rectangle (1.59,0.72 ); 


\fill[newgreen,  thick] (1.61,0) rectangle (1.71,0.33 ); 


\fill[newgreen,  thick] (1.73,0) rectangle (1.83,0.85 ); 


\fill[newgreen,  thick] (1.85,0) rectangle (1.95,0.345 ); 

\fill[newgreen,  thick] (1.97,0) rectangle (2.07,0.65 ); 

\fill[newgreen,  thick] (2.09,0) rectangle (2.19,0.74);
\fill[newgreen,  thick] (2.21,0) rectangle (2.31,1 ); 



\draw[-stealth, color=gray, thick] (0,0) -- (2.5,0);
\draw[-stealth, color=gray, thick] (0,0) -- (0,1.5);


\end{scope}

\end{tikzpicture}

\end{center}
   \caption{Illustration of a temporal action segmentation pipeline. Our dynamic clustering algorithm can be used for the second and third stages. \label{overview}}
\label{fig:short}
\end{figure*}

